SHViT: Single-Head Vision Transformer with Memory Efficient Macro Design

Recently, efficient Vision Transformers have shown great performance with low latency on resource-constrained devices. Conventionally, they use 4x4 patch embeddings and a 4-stage structure at the macro level, while utilizing sophisticated attention with multi-head configuration at the micro level. This paper aims to address computational redundancy at all design levels in a memory-efficient manner. We discover that using larger-stride patchify stem not only reduces memory access costs but also achieves competitive performance by leveraging token representations with reduced spatial redundancy from the early stages. Furthermore, our preliminary analyses suggest that attention layers in the early stages can be substituted with convolutions, and several attention heads in the latter stages are computationally redundant. To handle this, we introduce a single-head attention module that inherently prevents head redundancy and simultaneously boosts accuracy by parallelly combining global and local information. Building upon our solutions, we introduce SHViT, a Single-Head Vision Transformer that obtains the state-of-the-art speed-accuracy tradeoff. For example, on ImageNet-1k, our SHViT-S4 is 3.3x, 8.1x, and 2.4x faster than MobileViTv2 x1.0 on GPU, CPU, and iPhone12 mobile device, respectively, while being 1.3% more accurate. For object detection and instance segmentation on MS COCO using Mask-RCNN head, our model achieves performance comparable to FastViT-SA12 while exhibiting 3.8x and 2.0x lower backbone latency on GPU and mobile device, respectively.

==> Table/mobile_latency.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\begin{tabular}{lcl}
\hline
\multicolumn{1}{c}{\multirow{2}{*}{Model}} & Mobile Latency & \multicolumn{1}{c}{Top-1} \\
\multicolumn{1}{c}{}                       & (ms)           & \multicolumn{1}{c}{(\%)}  \\ \hline
E.Former-L1                                & 1.5            & 77.3 (79.2)               \\
E.FormerV2-S1                              & 1.3            & 77.9 (79.0)               \\
M.ViTv2 x1.0                               & 3.8            & 78.1                      \\
E.Net-B1                                   & 1.8            & 79.1                      \\
FastViT-T2                                 & 1.4            & 79.1 (80.3)               \\
M.One-S4                                   & 1.7            & 79.4                      \\
SHViT-S4                                   & 1.6            & 79.4 (80.0)               \\ \hline
\end{tabular}
\end{table}

==> checklist.tex <==
\newpage
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}

  
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}

  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{See Section~\ref{contribution}.}
    
  \item Did you describe the limitations of your work?
    \answerYes{See Section~\ref{conclusion}.}
    
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{See Section~\ref{intro}.}
    
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
    
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{See Section~\ref{assumptions}.}
    
	\item Did you include complete proofs of all theoretical results?
    \answerYes{See Section~\ref{sec:derivation}.}
    
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{The code is in the supplemental material. The data can be refered to Section~\ref{dataset}}
    
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
  \answerYes{See Section~\ref{dataset} and~\ref{imple_detail}.}
    
    \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNA{}
    
    \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See Section~\ref{imple_detail}.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}

  \item If your work uses existing assets, did you cite the creators?
    \answerYes{See Section~\ref{dataset}.}
    
  \item Did you mention the license of the assets?
    \answerNA{}
    
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
    
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
    
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
    
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
    
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}
\end{enumerate}
